Iterative Residual Policy: for Goal-Conditioned Dynamic Manipulation of Deformable Objects

This paper tackles the task of goal-conditioned dynamic manipulation of deformable objects. This task is highly challenging due to its complex dynamics (introduced by object deformation and high-speed action) and strict task requirements (defined by a precise goal specification). To address these challenges, we present Iterative Residual Policy (IRP), a general learning framework applicable to repeatable tasks with complex dynamics. IRP learns an implicit policy via delta dynamics -- instead of modeling the entire dynamical system and inferring actions from that model, IRP learns delta dynamics that predict the effects of delta action on the previously-observed trajectory. When combined with adaptive action sampling, the system can quickly optimize its actions online to reach a specified goal. We demonstrate the effectiveness of IRP on two tasks: whipping a rope to hit a target point and swinging a cloth to reach a target pose. Despite being trained only in simulation on a fixed robot setup, IRP is able to efficiently generalize to noisy real-world dynamics, new objects with unseen physical properties, and even different robot hardware embodiments, demonstrating its excellent generalization capability relative to alternative approaches. Video is available at https://youtu.be/7h3SZ3La-oA

==> text/old/evaluation.tex <==
\section{Evaluation}


\subsection{Metrics}
We measure the algorithm performance using distance to the goal (in cm) at each step \ben{(lower is better)}. \ben{ \sout{The faster an algorithm reaches a certain distance the better.}} Note that the pixel size is around 1.6cm in our trajectory image encoding and 0.7cm in \ben{the} real world tracking image.



\subsection{Ablation Study in Simulation}

\textbf{Setup} We compare different variations of our method as well as some baseline methods to show the efficacy of our method in simulation. We randomly sampled 5 ropes for both interpolation and extrapolation part of the test set with respect to the training set. For each rope, we randomly sampled 25 goals that is guaranteed to be reachable. For each trial, iterative algorithms run for 16 steps. The distance to the goal (in cm) averaged for each step across all goals and ropes is reported in fig. \ref{fig:sim}.

\textbf{Benefit of Implicitly Capturing System Parameters}
One obvious approach to this task is to first identify key system parameters, and then compute the optimal action to the goal using the identified parameters. We give this baseline a head start by providing the true varying parameters: length and density. To ensure fairness, we assume 16 fixed system identification actions are executed (equal to the maximum amount of information known by our method), and the resulting 16 trajectories are provided as input. We train a ResNet-50 network using the 16 trajectory images to regress the rope parameters. Another 4-layer MLP neural network, that takes in the rope parameter and goal, is trained to regress the action using optimal actions computed by brute-force on the training dataset. As shown in orange, labeled as "sysid" in fig. \ref{fig:sim}, it averages 10.4 cm error for interpolation ropes and 24.8 cm error for extrapolation ropes, significantly under-performs our method. Even if we assume we know the test rope parameter perfectly, as shown in brown and labeled as "plan" in fig. \ref{fig:sim}, the performance improvement is marginal. \shuran{what is the conclusion??}

\textbf{benefit of residual formulation }
Single step, delta action, but 

\textbf{Effect of action representation.}
Instead of \ben{\sout{representing} providing} delta actions as input to the network, and sampl\ben{\sout{e}ing candidate} delta actions at test time, \ben{\sout{here we will let the} we instead use a} network to directly regress \ben{the} optimal delta action. We train a ResNet-50 network, taking the current trajectory image and the goal (represented as a one-hot image) to regress the delta action, trained using brute-force computed optimal action on the training set. This iterative algorithm is initialized using the same action as our algorithms, and it's step size multiplied with a tuned proportional gain. As shown in pink and labeled "action\_direction", this method yields 4.6cm and 9.8cm error in the final step on interpolation and extrapolation ropes respectively. \ben{Ben: I would explicitly remind readers of the implicit action performance here too. These numbers don't mean much without a comparison.}

\textbf{Benefit of Adaptive Action Sampling.}
Inspired by proportional control, we compute the \ben{\sout{sigma} variance} of the action sampling Gaussian distribution by multiplying the current distance to the goal with a constant gain. Without this feature, shown in grey and labeled "const\_sigma" in fig. \ref{fig:sim}, the algorithm has difficulty converging to the optimal action. \ben{Ben: Discuss why?}

\textbf{Heuristic Baseline.}
\ben{Ben: I wouldn't phrase it like this. I think something like "to provide context for the performance of our approach, we compare against a trivial heuristic strategy:" ...}
One might argue that our algorithm has learned a trivial strategy: decrease both the speed and amplitude of the action if the goal is in between the trajectory and the origin (i.e. inside the trajectory) and increase both if otherwise. As shown in green and labeled "heuristic" in fig. \ref{fig:sim}, this heuristic policy converges very slowly on extrapolation ropes and diverges on interpolation ropes. Note that the step size of this heuristic policy is also proportional to the error, and the gain has been tuned for the optimal result. \shuran{why it doesn't work}

\subsection{Real World Evaluation}
\textbf{Experiment Setup.}
To test our method's generalizability against the sim-to-real gap, we \ben{\sout{tested} evaluated} our method on 9 different real-world setups. We tested a thin cotton rope (13g/m) of 3 different lengths (75cm, 100cm, 125cm), a thick cotton rope (65g/m, 1m in length), a leather bullwhip (72g/m, 1m in length) and a piece of red cloth (1m in length). We modeled the simulation rope after the thin cotton rope, therefore other ropes \ben{\sout{should be considered} are significantly} out-of-distribution. In particular, the red cloth \ben{---} due to much larger surface area to density ratio \ben{---{} behaves very differently from a typical rope. }

\shuran{it is method not evaluation}
To obtain the rope tip trajectory as an input of our algorithm, we trained a tracking model based on DeeplLabV3+ with 400 hand labeled images. The tracking error on the validation set is 1.8 pixels, which translates to 1.3 cm for our setup. 

To speedup the data collection process, we terminate the algorithm once the error has reached 1.6 cm.


\textbf{Sim2Real Adaptation.}
The evaluation result has been summarized in Tab. \ref{tab:real_eval}. We compare against 2 baselines. NN: Optimal action (computed using brute force) for the nearest neighbor rope in terms of rope parameter. AVG: The action that minimizes the average distance to goal in the training set, regardless of rope parameter. Note that our method is initialized using this action. As shown in the Tab. \ref{tab:real_eval}, our method outperforms both baseline by a significant margin, and is very close to the tracking error. This result is particularly impressive for the red cloth. More details about of each steps of our algorithm has been shown in Fig. \ref{fig:real_detail}.
\shuran{point you want to make, iterative approach bridge the sim2real gap?}

\textbf{Online Adaptation.}
One advantage of using an interactive adjustment algorithm is the robustness against dynamic system changes. In this experiment, we first run the algorithm on the thin cotton rope (13g/m, 1m in length) for 6 steps. Just before step 7, we pause the robot and tie 3 knots that significantly changes the rope's length, density and mass distribution. As shown in Fig. \ref{fig:online_adaptation}, our algorithm quickly adjust\ben{ed} to the \ben{\sout{new} changed} system \ben{dynamics} and returned to the low error state. 


\begin{figure*}
    \centering
    \includegraphics[width=0.66\linewidth]{figure/sim_plots.pdf} ~\includegraphics[width=0.3\linewidth]{figure/split_plot.pdf}
    \caption{\textbf{Simulation Evaluation.} Distance to goal in cm averaged across 5 ropes and 25 goals for each method, shown with 95\% confidence interval. Test rope parameters that are extrapolation with respect to training ropes (right) yield higher errors in general comparing to interpolation (left). The result of single-step methods (sysid, plan) are shown as lines for visualization.
    
    \textbf{Dataset Split.} \shuran{train. test - interpolation. test - extrapolation} \shuran{Same Y axis limit}
    The $12\times12$ grid of rope parameters used for simulation. In total, there are $64,31,49$ ropes in the training,validation and testing set respectively.}
    \label{fig:sim}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/interrupt_plot.pdf}
    \caption{\textbf{Online Adaptation.} Error plot of our algorithm tested on a thin cotton rope. Just before step 7, we paused the experiment and tied 3 knots on the rope that significantly changed the rope's length, density and mass distribution. Our algorithm quickly adapted to this change in the system afterwards.}
    \label{fig:online_adaptation}
    % https://docs.google.com/drawings/d/113vNeGlj8giXRdVfd47gkosV1PIefxu8HKGWcSKNlh8/edit?usp=sharing
\end{figure}


\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{figure/mujoco_ur5.png}
    \caption{\textbf{MuJoCo simulation.} A UR5 robot swings a rope via an extension stick. The rope is modeled using 25 connected capsules.}
    \label{fig:mujoco}
\end{figure}


\begin{table}[]
    \begin{tabular}{lrrrr}
    \toprule
    {} &    NN &   AVG &  Ours Step3 &  Ours Step9 \\
    \midrule
    long\_stick\_thin\_red &  9.94 & 11.33 &        2.13 &        1.33 \\
    red\_cloth           & 26.72 & 30.43 &        7.00 &        0.99 \\
    short\_thin\_red      &  8.71 & 10.17 &        4.54 &        2.81 \\
    thick\_red           & 11.68 & 10.05 &        5.95 &        1.66 \\
    thin\_black          & 11.38 & 14.66 &        4.58 &        0.99 \\
    thin\_red            &  8.23 &  7.98 &        1.66 &        0.66 \\
    \bottomrule
    \end{tabular}
    % \begin{tabular}{lrrrrrr}
    % \toprule
    % {} &  long\_stick\_thin\_red &  red\_cloth &  short\_thin\_red &  thick\_red &  thin\_black &  thin\_red \\
    % \midrule
    % NN   &                 9.94 &      26.72 &            8.71 &      11.68 &       11.38 &      8.23 \\
    % AVG  &                11.33 &      30.43 &           10.17 &      10.05 &       14.66 &      7.98 \\
    % Ours &                 1.33 &       0.99 &            2.81 &       1.66 &        0.99 &      0.66 \\
    % \bottomrule
    % \end{tabular}
    \caption{\textbf{Real World Evaluation.} Distance to goal in cm in 6 real world ropes. red\_cloth and thin\_black are particularly out-of-distribution. NN: optimal action for most similar rope in the training set. AVG: action minimizes average error across all ropes in the training set. Ours: our method's error at step 3 and step 9.}
    \label{tab:real_eval}
\end{table}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/real_vis_plots.pdf}
    \caption{\textbf{Results.} Left error plot for ours and baseline. Right, first, 5th, and last action trajectory for \names~and baselines. 
    \todo{make the line color consistent, make sure trajectory is visible, show rope and robot only for ours, other baseline only show trajectory}
    More results can be find in supp videos. \shuran{all the images has a strange white balance} }
    %https://docs.google.com/drawings/d/1oiWSkWwh9zzMQ_cAMQME6a0cPVZw53zplIQvz1UpmLs/edit?usp=sharing
    \label{fig:real_detail}
\end{figure*}


\section{Conclusion} 
\label{sec:conclusion}

The conclusion goes here. \ben{Ben: It might be helpful to put a few bullets here before too much more gets added to the main document. What's the big takeaway here, why is this strategy effective
and how would you what are the important take-aways?}

==> text/old/introduction.tex <==
\section{Introduction}

\todo{} 

We are using the task of hitting targets precisely with a whip as a case study for dynamic manipulation of deformable object. This is a challenging task due to following factors: 
\begin{itemize}[leftmargin=3mm]

\item \textbf{Complex object properties:} Unlike \ben{a} rigid object, the motion of a deformable object is influenced by many more factors such as stiffness, aerodynamic, density distribution, where many of these parameters are notoriously difficult to model or measure. \shuran{missing the aspect of high dof, under-actuated}
Therefore, prior studies are often confined to known objects and fail to generalize to new objects with different properties. 

\item \textbf{Complex dynamics:} Unlike quasi-static manipulation, dynamic manipulation is ??  (action - trajectory, instead of action - position? ) %less predictable -- same action same rope can result in different trajectory due to different initial conditions. This uncertainty varies with respect to action, goal configuration and rope parameters, requiring the system to explicitly model this uncertainty and plan its action accordingly. 
\shuran{maybe this complex action object property relationship can be mentioned here?}
\ben{Ben: I think this misses some of the aspects that make deformable objects (and cloth in particular) so interesting and challenging. While cloths and whips have virtually infinite degrees of freedom in principle, at any given time the \textit{effective degrees of freedom} are highly dependant on the action being taken and contact between the object and environment. A whip moving at high speed in a circular motion is, for all intents and purposes, temporarily fully actuated and has essentially only 6 degrees of freedom (i.e. it's rigid). In contrast to rigid objects, dynamics affects not only the object's interaction with its environment but also the effective kinematics of the object itself.}


\item \textbf{Precise goal condition:}  Due to these challenges, prior works on dynamic deformable object manipulation focus tasks that has a lower precision requirement (e.g., cloth unfolding \cite{ha2021flingbot}, or cable vaulting \cite{zhang2021robots}). In contrast, our task require the system to produce accurate actions in order to precisely reaching goal condition (i.e., hitting the goal position with \the tip of a whip). \ben{Ben: I think this bullet conflates two things. 1: The how many distinct behaviors can achieve a goal and 2: How precise is the goal. It's possible that a very precise goal can still be achieved with multiple very different policies/strategies/trajectories.}

\end{itemize}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/rope-teaser.pdf}
    %https://docs.google.com/drawings/d/12tlTQ5S-eEHEXbHswpW1-dkgyWmvPPUlsDF5sNXWmwo/edit?usp=sharing

    \caption{(Place holder) Teaser Tasks, Realworld Robot + Rope figure.  highlight the iterative process, trajectory for step 1,2,3,4.  \todo{caption}
    }
    \label{fig:task}
\end{figure}


In this work, we present \textbf{\namel~(\names)}, an self-supervised formulation that learns how to plan control parameters for whipping a deformable rope  from visual observations. 
\todo{summary of how the system works}
This formulation highlight two key features: 
\begin{itemize}[leftmargin=3mm]
\item \textbf{Residual trajectory representation}: Instead of trying to capture the entire dynamical system and identify key physical parameters, \names~only learns how a given trajectory will deform under small changes in action. This formulation efficiently reuses the rich physical information captured by the observation, which allows the model to generalize to unseen ropes with significantly different dynamics comparing to training data.
\shuran{"reuses the rich physical information captured by the observation", why?}

\item \textbf{Iterative Action Improvement}: Instead of learning the direction mapping from the goal to the final action, \names~starts with an rope-agnostic action initialization and selects the best delta action sample that would lead towards the goal. The system then continues to readjust its actions base on the new observations. For tasks with repeatable actions, this iterative approach allows the system to achieve high precision and robust against errors from action, observation and model prediction.


% \item \textbf{Implicit system representation}: %what we do, what's the advantage. 
% Instead of explicitly model the object physical properties, \names~learns a implicit latent representation of the deformable object from a sequence of visual observation under dynamic interaction. This formulation allows the model to learn most relevant object feature representation through active interaction, which is more flexible than a set of predefined physical parameters and easier to adapt to new scenarios.  

% \item \textbf{Residual action inference:} %what we do, what's the advantage.
% Instead of learning the direct mapping from the goal to the final action, \names~starts with an random action initialization and infers delta action at each step that would lead towards the goal. The system then continues to readjust its actions base on the new observations. This iterative approach is what allows the system to achieve precise prediction and control for this highly dynamical and complex task, since predicting trajectory deviation for small delta action is much easier than memorizing trajectory for all possible actions.
\end{itemize}

This formulation provide a  general framework for precise dynamic manipulation that allows  efficient generalization for varying rope properties, robot hardware parameters.  Thanks to its adaptable formulation, the model trained in simulation can be directly applied to realworld robot platform with online adaptation.  

In summary, our  primary contribution is the \namel~(\names), an self-supervised formulation that learns how to plan control parameters  for dynamically manipulating (whipping) a deformable rope  from visual observations. 
We demonstrate this framework in the task of xxx. 
Our experiment shows ... 


\iffalse
\textbf{Problem:}
\begin{itemize}    
    \item{Difficult to model dynamics}: High degrees of freedom with non-linear dynamics and difficult to measure parameters. \textbf{Hard to compute Jacobian analytically.} This makes model-based control/RL difficult. \textbf{Large sim-to-real gap.}
    
    \item{Difficult to plan/control}: Highly underacutated. Goal can not be mapped trivially to actions.
\end{itemize}

\textbf{Solution:}
\begin{itemize}
    \item{Learning the notion of Jacobian} for \textbf{online adaptation}. Intuitive physics.
    \item{Identical input and output representation} easier to learn, better generalization.
    \item{Motion primitive} to reduce action space.
\end{itemize}

\textbf{Contribution:}
\begin{itemize}
    \item{First to solve a task} Goal conditioned dynamic manipulation of deformable.
    \item{A method to close the sim-to-real gap} Representation to enable online adaptaion.
\end{itemize}

\textbf{Key takeaway:}
\begin{itemize}
    \item{Learned close-loop policy transfer better}
    \item{Decouple goal and learning}
    \item{}
\end{itemize}


% Current literature interpreters the term intuitive physics in different ways. 
% 1. Object permance
% 2. Learning output of physics simulation or residual
% 3. Predict next state given current state and action

% Our work is more in-line with clever reformulation of the original problem for easier learning.
% And turn problem into class 3.
\fi 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.49\linewidth]{example-image-golden}~\includegraphics[width=0.49\linewidth]{example-image-golden}
    \caption{Challenges: (1) Show trajectory of whipping 3 different rope with same action (different stiffness, mass distribution) (2) Same rope same action, executed in 10 times, show the averaged trajectory for uncertainty (? if we don't handle uncertainty, don't include this). }
    \label{fig:task}
\end{figure*}
